Universal Domain Adaptation through Self Supervision

Unsupervised domain adaptation methods traditionally assume that all source categories are present in the target domain. In practice, little may be known about the category overlap between the two domains. While some methods address target settings with either partial or open-set categories, they assume that the particular setting is known a priori. We propose a more universally applicable domain adaptation framework that can handle arbitrary category shift, called Domain Adaptative Neighborhood Clustering via Entropy optimization (DANCE). DANCE combines two novel ideas: First, as we cannot fully rely on source categories to learn features discriminative for the target, we propose a novel neighborhood clustering technique to learn the structure of the target domain in a self-supervised way. Second, we use entropy-based feature alignment and rejection to align target features with the source, or reject them as unknown categories based on their entropy. We show through extensive experiments that DANCE outperforms baselines across open-set, open-partial and partial domain adaptation settings. Implementation is available at https://github.com/VisionLearningGroup/DANCE.

==> figures/entropy_separation.tex <==

\begin{figure}[t]
    \centering
    \vspace{-0.15mm}
    \includegraphics[width=\linewidth]{imgs/ent_sep.jpg}
    \vspace{-9mm}
    \caption{\small An overview of the entropy separation loss (best viewed in color). We further decrease small entropy to move the sample to a ``known"-class prototype, and increase large entropy to move it farther away. Since distinguishing ``known" vs ``unknown"  samples near the boundary is hard, we introduce a confidence threshold that ignores such ambiguous samples.}
    \label{fig:overview}
\end{figure}

==> figures/neighborhood_clustering.tex <==

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{imgs/clustering2.jpg}
     \vspace{-7mm}
    \caption{Similarity distribution calculation in neighborhood clustering (best viewed in color). We minimize the entropy of the similarity distribution between each point (as shown for $f_1$), the prototypes, and the other target samples. Since most target samples are absent in the mini-batch, we store the their features in a memory bank, updating it with each batch.
    }
    \label{fig:ent}
\end{figure}

==> figures/setting.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{imgs/dance_fig1.pdf}
     \vspace{-7mm}
    \caption{Unlike previous methods tailored to each setting, our proposed approach, called DANCE, performs well on all sub-settings of universal domain adaptation.} 
    \label{fig:setting}
\end{figure}

==> intro2.tex <==
\section{Introduction}
Deep neural networks can learn highly discriminative representations for image recognition tasks~\cite{imagenet, simonyan2014very, krizhevsky2012imagenet, faster, maskrcnn}, but do not generalize well to domains that are not distributed identically to the training data. Domain adaptation (DA) aims to transfer representations of source categories to novel target domains without additional supervision. Recent deep DA methods primarily do this by minimizing the feature distribution shift between the source and target samples~\cite{ganin2014unsupervised, long2015learning, sun2015return}. However, these methods make strong assumptions about the degree to which the source categories overlap with the target domain, which limits their applicability to many real-world settings.
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{imgs/dance_fig1.pdf}
     \vspace{-7mm}
    \caption{Unlike previous methods tailored to each setting, our proposed approach, called DANCE, performs well on all sub-settings of universal domain adaptation.} 
    \label{fig:setting}
\end{figure}

In this paper, we address the problem of \textit{Universal DA}. Suppose $L_s$ and $L_t$ are the label sets in the source and target domain. In Universal DA we want to handle all of the following potential ``category shifts": closed-set ($L_s=L_t$), open-set ($L_s \subset L_t$)~\cite{busto2017open,saito2018open}, partial ($L_t \subset L_s$)~\cite{cao2018partial}, or a mix of open and partial~\cite{UDA_2019_CVPR}, see Fig.~\ref{fig:setting}. Existing DA methods cannot address Universal DA well because they are each designed to handle just one of the above settings. 
However, since the target domain is unlabeled, we may not know in advance which of these situations will occur. Thus, an unexpected category shift could lead to catastrophic misalignment. For example, using a closed-set method when the target has novel (``unknown'') classes could incorrectly align them to source (``known'') classes.
The underlying issue at play is that existing work heavily relies on prior knowledge about the category shift.

The second problem is that the over-reliance on supervision in
the source domain also makes it challenging to obtain discriminative features on the target.
 \begin{figure*}[!h]
    \centering
    \includegraphics[width=\linewidth]{imgs/fig1.pdf}
    \vspace{-9mm}
    \caption{    
    We propose \textit{DANCE}, which combines a self-supervised clustering loss \textcolor{red}{(red)} to cluster neighboring target examples and an entropy separation loss \textcolor{gray}{(gray)} to consider alignment with source (best viewed in color).}
    \label{fig:fig1}
\end{figure*}
Prior methods focus on aligning target features with source, rather than on exploiting structure specific to the target domain. 
In the universal DA setting, this means that we may fail to learn features useful for discriminating ``unknown'' categories from the known categories, because such features may not exist in the source. 

Self-supervision was proposed in~\cite{carlucci2019domain} to extract domain-generalizable features, but it is limited in extracting discriminative features on the target. 
 
We propose to overcome these challenging problems by introducing \textit{Domain Adaptive Neighborhood Clustering via Entropy optimization (DANCE)}. An overview is shown in Fig.~\ref{fig:fig1}. Rather than relying only on the supervision of source categories to learn a discriminative representation, \textit{DANCE} harnesses the cluster structure of the target domain using self-supervision. This is done with a ``neighborhood clustering" technique that self-supervises feature learning in the target. At the same time, useful source features and class boundaries are preserved and adapted with a partial domain alignment loss that we refer to as ``entropy separation loss." This loss allows the model to either match each target example with the source, or reject it as an ``unknown'' category. 
 
Our contributions are summarized as follows:
\begin{itemize}
\vspace{-.4cm}
    \item We propose  \textit{DANCE}, a universal domain adaptation method that can be applied out-of-the-box without prior knowledge of specific category shift, 
    \vspace{-.2cm}
    \item We experimentally observe that \textit{DANCE} is the only method that outperforms the source-only model in every setting, 
    \vspace{-.2cm}
    \item We achieve state-of-the-art performance on all open-set and open-partial DA settings, and some partial DA settings, and
    \vspace{-.2cm}
    \item We learn discriminative features of ``unkown'' target samples even without any supervision. 
  \end{itemize}
  

==> introduction.tex <==
\section{Introduction}
\vspace{-5mm}
%\donghyun{I think it could be better to separate notions between "domain gap" and "category gap" for clarity}
%Recently,  deep convolutional networks that learn rich feature representations have boosted the accuracy of many image recognition task~\cite{imagenet, simonyan2014very, krizhevsky2012imagenet, faster, maskrcnn}. 
%However, we need to collect a lot of annotated examples to train the model.
%One way to reduce the cost of the annotation is transferring knowledge obtained in a label-rich domain to the label-scarce domain. Domain adaptation is one of the research fields to tackle the challenge. We have a label-rich domain called source and a label-scarce domain called target. 
%The goal is to train a model working well on the target domain. 
%Unsupervised domain adaptation (UDA) assumes that all of the examples in the target domain are unlabeled. UDA is very challenging and a practical problem to reduce annotation cost. The goal of domain adaptation is to extract discriminative target features that are useful for classification. 

%There are two difficulties in this task. First, each domain has distinct characteristics in the style or appearance of the image features, which can worsen the performance of a learned model. The second difficulty is a category shift, where some categories are shared across domains while others are not. 
%For example, we tackle the first difficulty in closed domain adaptation where we have the same classes across two domains. A representative solution is a distribution matching with a domain classifier~\cite{ganin2014unsupervised}. To extract discriminative target features, we train a model to align target features with source.
%Recently, various category-shift settings and corresponding methods have been proposed to tackle both first and second difficulties. 
%For example, open-set domain adaptation (ODA)~\cite{busto2017open, saito2018open} deals with the situation where the target domain contains categories absent in the source domain.
%Partial domain adaptation (PDA)~\cite{cao2018partial}, where the target domain contains the subset of source classes, is also a popular task. Besides, universal domain adaptation (UDA)~\cite{UDA_2019_CVPR} is the combination of partial domain adaptation and open-set domain adaptation. When there are both feature characteristic-gap and category-gap between source and target, the task can be very challenging. Domain classifier based method is adjusted to solve each specific task and shown to perform well~\cite{saito2018open, cao2018partial, UDA_2019_CVPR}. 

%A representative solution is a distribution matching based approach. To reduce the domain-gap in the feature space, we train a model to minimize the feature distribution distance. Since target domain examples are not annotated, the assumption of completely sharing categories may not be realistic.
%Then, open-set domain adaptation~\cite{busto2017open, saito2018open} is recently proposed, where the target domain contains categories absent in the source domain. The model has to detect out-lier target examples as well as to classify known target examples. The challenge of the task is that if we strongly align target feature distribution with source one, the model will fail to detect unknown examples. 
%Partial domain adaptation~\cite{cao2018partial}, where the target domain contains the subset of source classes, is also a popular task. 
%Besides, universal domain adaptation~\cite{UDA_2019_CVPR} is proposed, which is the combination of partial domain adaptation and open-set domain adaptation. 
%\donghyun{just mentioning 'various setting' may be confusing.}
%However, an important challenge is that the target domain can be a black-box because it is an unlabeled domain. We may not be able know which methods to apply to an unlabeled target domain. 
%All methods are designed to deal with each task and it is questionable whether they work well on the other tasks. UDA is proposed to handle mixture of all tasks, but they applied their method only to the mixture of them. In this paper, our goal is to solve all tasks above with a single method without optimizing a method for each setting. This setting is very challenging and practical.

%The problem of existing methods is that they are designed to strongly rely on the prior knowledge about the categories shared by source and target. For example, the distribution alignment methods try to align target examples with source~\cite{ganin2014unsupervised, long2015learning, sun2016deep} because we can extract discriminative target features by aligning with the labeled domain's feature. 
%They assume that target and source domain share categories .
%Therefore, when the assumption does not hold, the methods can significantly fail. For example, if we apply a simple distribution alignment to ODA setting, unknown target classes can be aligned with known source classes. In addition, several ODA methods assumes that there are some proportion of unknown target examples. If the target domain shares the category with source, they will fail in adaptation. 

%To avoid such a negative transfer, we propose to utilize the cluster structure of the target domain, namely, self-supervision in the target domain. By clustering neighboring target examples, we can extract discriminative target features. Since the clustering is designed not to rely much on source examples, our method robust to the category-shift between source and target. 

%Our main idea is to extract discriminative target features by clustering neighboring target examples together. By doing that, examples having similar features can be better clustered with each other. Since we utilize cluster structure in the target domain, we do not have to rely too much on the relationship between source and target, which can make our method robust to the category-gap between source and target. 
%In addition, we need to consider whether to align the target examples with source in a category-shift robust way. To achieve the goal, we propose an entropy-separation loss. With respect to the known classification output, entropy of unknown examples should be large whereas that of known ones should be small. Following this assumption, we propose to make the target examples have entropy value separated from a certain value and achieve both alignment and rejection. 

%We show that combining two losses work well on various domain adaptation settings.

Deep learning models perform very well on various image recognition tasks~\cite{imagenet, simonyan2014very, krizhevsky2012imagenet, faster, maskrcnn}, but we require a large amount of labeled data to train them. 
Domain adaptation (DA) leverages unlabeled data collected from the target domain in addition to labeled data from the source domain. 
The main problem in DA is the domain shift. The source and target domain have different characteristics in their appearance or texture. 
State-of-the-art domain adaptation methods solve the problem by aligning target features with source ones~\cite{ganin2014unsupervised, long2015learning, sun2015return}. There are two overlooked problems in current methods.
\input{figures/setting}

%We believe that DA should be truly universally applicable in that it works without exact knowledge of the target classes. 


First, since the target domain is unlabeled, it can have various kinds of categories different from the source domain, as shown in Fig. \ref{fig:setting},  open-set~\cite{busto2017open,saito2018open}, partial~\cite{cao2018partial}, open-partial domain adaptation~\cite{UDA_2019_CVPR} (ODA, PDA, OPDA), which we call category shift. Changing methods or hyperparameters according to the category shift is hard because we cannot know the shift in an unlabeled target domain. Therefore, we need a method performing well on diverse category shifts without changing hyperparameters.
%\donghyun{The problem of “without changing hyperparameters” should come first. Otherwise, it is not clear why “without changing hyperparameters” is good. Can we first say that existing methods tune hyper-parameters by accessing the unlabled target examples? } 
However, most prior work ignores this, assumes a specific set of categories and designs a method specialized in each setting. The difficulty is that a catastrophic misalignment can occur when an unexpected category-shift happens. For example, if we apply a simple distribution alignment to ODA where we have unknown target classes, they can be aligned with known source classes (top of Fig. \ref{fig:fig1}). The underlying issue is that prior methods rely a lot on the supervision of the source domain and the prior knowledge about the category-shift. We call the first problem \textit{universal shift}.

Second, extracting discriminative features for the unknown target classes is hard because of the same reason. Aligning target samples with the source makes it hard to exploit cluster structure specific to the target domain.
However, obtaining the discriminative representations is useful when we aim to classify unknown classes into the correct categories. We call the second problem \textit{unknown class clustering}.


In this paper, we propose a method that solves the two challenging problems. The overview is described at the bottom of Fig. \ref{fig:fig1}.
We propose Domain Adaptive Neighborhood Clustering via Entropy optimization (DANCE), which have two components. 
First, we perform clustering target samples using self-supervision in the target domain. The cause of \textit{universal shift} and \textit{unknown class clustering} is that existing methods rely a lot on the source domain. Instead, we harness the cluster structure of the target domain. We extract discriminative features for both known and unknown categories by effectively using self-supervision in the target domain. We call the method neighborhood clustering.
Second, to classify them correctly, we propose a weak alignment, which we call entropy separation loss. We train a model to choose either match each target example with the source or reject it as unknown categories. 
Combining both components solve \textit{universal shift} whereas
\textit{unknown class clustering} is solved by neighborhood clustering.


Our contribution is summarized as follows, 
\begin{itemize}
    \item We proposed DANCE, which deals with universal domain shift.
    \item We observe that our method is the only method outperforms the source-only model in every setting. %
    \item Our method achieved state-of-the-art performance on all open-set and open-partial adaptation, and a part of partial domain adaptation settings. 
    \item The features learned by our method are also effective to classify unknown classes into correct classes. 
  \end{itemize}
   
%\textbf{Recommended text starting from second paragraph}
%\donghyun{
%We tackles the problem of universal domain adaptation (UDA) where no prior knowledge on category-shift is known. Fig. \ref{fig:setting} describes our goal, which we propose a method that can handle all different types of category-shift, including open-set (ODA)~\cite{busto2017open,saito2018open}, partial (PDA)~\cite{cao2018partial}, universal domain adaptation (UDA)~\cite{UDA_2019_CVPR}.  

%Prior methods overlook are three major problems in DA. \textbf{First}, existing methods are designed for each specific category-shift. Since the target domain is an unlabeled domain, we are not able to types of category-shift between source and target domain in advance. In addition hyperparameters are tailored to each adaptation scenario, which we are not able to accomplish in the real world. A method should work on the diverse kinds of class distribution shifts without tuning hyperparameters for each adaptation scenario. 
%\textbf{Second}, since most methods are designed for a specific category-shift setting, catastrophic misalignment can happen under a different category-shift. For example, if we apply a simple distribution alignment to ODA where we have unknown target classes, they can be aligned with known source classes (Upper in Fig. \ref{fig:fig1}). A similar negative transfer can happen in the case of PDA and UDA. The underlying issue is that prior methods rely a lot on the supervision of the source domain and the prior knowledge about the category-shift. 
%\textbf{Third}, extracting discriminative features for the unknown target classes is hard because existing ones rely a lot on the supervision of the source domain. However, obtaining the discriminative representations of unknown examples is desired when we aim to identify unknown classes.  In this paper, we propose a method that solves the three challenging problems. The overview is described in the bottom of Fig. \ref{fig:fig1}.

%We propose two novel components. First, we perform clustering target examples using self-supervision in the target domain. The cause of the problems is they assumed a specific relationship between domains. We need to exploit the cluster structure of the target domain. We extract discriminative features for both known and unknown categories by effectively using self-supervision in the target domain.
%Second, we propose a weak alignment objective to the source domain. The first objective will give us well-clustered target features. To classify them correctly, we need to choose either match them with the source or reject them as unknown categories. \donghyun{Clear enough?}

%Our contribution is summarized as follows, 
%\begin{itemize}
%    \item We proposed UDAS, which deals with universal domain shift without any prior knowledge.
%    \item Our method achieved state-of-the-art performance on all open-set and universal domain adaptation, and a part of partial domain adaptation settings. 
%    \item Our method improved the performance compared to source-only model in every setting without exhaustive hyper-parameter tuning for each setting. \donghyun{more expressive word may needed rather than 'without chaning hyper-parameter'} \donghyun{before looking experimental section, does beating source-only model sound impactful to reviewer?}
%    \item The features learned by our method is also effective to classify unknown classes into correct classes. 
%   \end{itemize}


\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{imgs/fig1.pdf}
    \vspace{-7mm}
    \caption{An overview of our method (Best viewed in colors). Top: Conventional distribution alignment can fail in open set domain adaptation. Bottom: We propose self-supervised clustering loss \textcolor{red}{(red)} to cluster neighboring target samples and entropy separation loss \textcolor{gray}{(gray)} to consider alignment with source.}
    \label{fig:fig1}
\end{figure*}
%}

%An overlooked problem in DA is that in many scenarios the target domain could have a different distribution of classes. Since the target domain is an unlabeled domain, the target domain can have different classes from the source.
%However, most prior work ignores this and assumes a closed set of categories and tries to simply aligns all target points to source ones. 
%Recently, some work attempted to take the category gap into account: open-set~\cite{busto2017open,saito2018open}, partial~\cite{cao2018partial}, universal domain adaptation~\cite{UDA_2019_CVPR} (ODA, PDA, UDA) were proposed. ODA considers the situation where target domain contains unknown classes absent in the source. PDA considers the source classes absent in the target domain. UDA is the mixture of ODA and PDA. 
%The general problem of existing methods is that they are designed to strongly rely on prior knowledge about the categories shared by source and target. For example, the distribution alignment methods try to extract discriminative target features by aligning target examples with the source. This means that they assume the relationship that target and source domain share categories. Therefore, when the assumed relationship does not hold, the methods can significantly fail. For example, if we apply a simple distribution alignment to ODA, unknown target classes can be aligned with known source classes. A similar negative transfer can happen in the case of PDA and UDA. 
%Specifically, UAN~\cite{UDA_2019_CVPR} employed importance weighted domain classifier to partially align target example with source for UDA setting. The method has three problems; (1) they applied it only to UDA. (2) it cannot learn discriminative features for unknown categories. (3) since they do not have objective to learn to reject unknown example, all target features are aligned with source to some extent. 

%We believe DA should be truly universally applicable and work without exact knowledge of the target classes. Under this assumption, the method should work without tuning hyper-parameters for each setting. If we can tune them, we can choose hyper-parameters such as the threshold value to reject unknown examples, which violates the assumption of universal applicability. 
%Although this is a very challenging setting, we propose a method that has this property. 
%The key is not to rely a lot on aligning the two entire domains together to extract discriminative target features. 
%Instead, we propose two novel components for target examples; self-supervised clustering and entropy-based alignment with a rejecting option. In addition, we utilize the property of batch normalization. Overview is described in Fig.~\ref{fig:fig1}.
%First key idea is to move points closer together (self supervision) and obtain better clustered target features. This clustering allows us to extract discriminative features even for classes present only in target domain. To achieve it, we perform entropy minimization on similarity distribution among unlabeled target examples and prototypes of source examples. 
%Second, we propose a way to align the target features with the source or to reject as unknown. We use the classifier’s output to calculate entropy and train the model to either increase or decrease the entropy, which we call entropy separation. If the entropy is small, the example should be aligned with a source known class, then we decrease the entropy. By contrast, if it is large, the example should be kept far from the source, then we increase the entropy. We use the entropy to decide unknown or known in the test time. 
%In addition, we utilize the effect of domain-specific batch normalization (BN) to weakly align feature distributions between source and target domain~\cite{li2016revisiting, chang2019domain, saito2019semi}. We forward the mini-batches of different domains separately. Thus, domain-specific features can be reduced. 



==> supple_arxiv.tex <==
%\donghyun{What about using the tables and figures in supplementary as Alphabet instead of number used in the main paper?}

\begin{table*}[]
\begin{center}
\scalebox{0.62}{
\begin{tabular}{c|cc|cc|cc|cc|cc|cc||cc|cc|cc|cc|cc|cc}
\toprule[1.5pt]
&\multicolumn{12}{c||}{Open Set}&\multicolumn{12}{|c}{Open Partial}\\\hline
\multirow{2}{*}{Method}&\multicolumn{2}{c|}{A to W}        & \multicolumn{2}{c|}{D to W}    & \multicolumn{2}{c|}{W to D}      & \multicolumn{2}{c|}{A to D}     &\multicolumn{2}{c|}{D to A}      & \multicolumn{2}{c||}{W to A} & \multicolumn{2}{c|}{A to W}        & \multicolumn{2}{c|}{D to W}    & \multicolumn{2}{c|}{W to D}      & \multicolumn{2}{c|}{A to D}     &\multicolumn{2}{c|}{D to A}      & \multicolumn{2}{c}{W to A}       \\\cline{2-25}
 & OS   & OS*    & OS   & OS*    & OS   & OS*    & OS   & OS*    & OS   & OS*    & OS   & OS*    & OS   & OS*    & OS   & OS*    & OS   & OS*    & OS   & OS*    & OS   & OS*    & OS   & OS*   \\\hline
SO   & 83.8 & 87.7 & 95.3 & 99.0  & 95.3 & 100.0 & 89.6 & 93.6 & 85.6 & 86.3 & 84.9 & 88.2 & 75.7 & 79.2 & 95.4 & 98.1 & 95.2 & 100.0 & 83.4 & 88.3 & 84.1 & 84.9 & 84.8 & 85.7 \\
DANN & 87.6 & 95.7 & 90.5 & 99.3  & 91.2 & 100.0 & 88.7 & 96.9 & 87.4 & \bf{95.4} & 87.0 & 95.2 & 83.0 & 90.0 & 89.3 & 97.1 & 89.5 & 96.9  & 81.9 & 88.8 & 80.2 & 86.8 & 78.2 & 77.8 \\
%MDD  & 0.0  & 0.0  & 0.0  & 0.0   & 0.0  & 0.0   & 0.0  & 0.0  & 0.0  & 0.0  & 0.0  & 0.0  & 0.0  & 0.0  & 0.0  & 0.0  & 0.0  & 0.0   & 0.0  & 0.0  & 0.0  & 0.0  & 0.0  & 0.0  \\
ETN & 86.7 & 95.4 & 90.0 & 99.0  & 90.1 & 99.1  & 89.1 & 98.0 & 86.7 & 95.3 & 86.6 & 95.3 & 89.1 & \bf{98.0} & 90.6 & \bf{99.7} & 90.9 & \bf{100.0} & 86.3 & \bf{94.9} & 86.4 & \bf{95.0} & 86.5 & \bf{95.1} \\
STA & 91.7 & 94.6 & 94.4 & 98.1  & 94.8 & 100.0 & 90.9 & 94.2 & 87.3 & 88.8 & 80.6 & 82.4 & 85.2 & 87.8 & 96.3 & 99.1 & 95.1 & 100.0 & 88.1 & 90.6 & 87.9 & 88.7 & 86.0 & 87.1 \\
UAN& 86.2 & 94.6 & 89.5 & 98.5  & 90.2 & 99.2  & 89.8 & 98.7 & 85.8 & 94.4 & 84.2 & 92.7 & 78.8 & 86.7 & 83.5 & 91.9 & 84.9 & 93.4  & 77.5 & 85.3 & 75.7 & 83.3 & 75.6 & 83.1 \\
Ours & \bf{93.6} & \bf{97.2} & \bf{97.0} & \bf{100.0} & \bf{97.1} & \bf{100.0} & \bf{95.7} & \bf{98.4} & \bf{91.0} & 94.9 & \bf{90.3} & \bf{95.6} & \bf{92.8} & 96.4 & \bf{97.8} & 99.1 & \bf{97.7} & 99.6 & \bf{91.6} & 94.0 & \bf{92.2} & 94.5 & \bf{91.4} & 94.7\\
 \bottomrule[1.5pt]
\end{tabular}
}
\caption{Evaluation on two metrics on open-set and open partial domain adaptation. OS is average of all classes. OS* is the average of known classes.}
\label{tb:oda_opada}

\end{center}
\end{table*}

\begin{table*}[]
\begin{center}

\scalebox{0.7}{
\begin{tabular}{c|ccccccccccccc}
\toprule[1.5pt]
Setting  &Ar2Cl                    & Ar2Pr & Ar2Rw & Cl2Ar & Cl2Pr & Cl2Rw & Pr2Ar & Pr2Cl & Pr2Rw & Rw2Ar & Rw2Cl & Rw2Pr & Avg      \\\hline
CDA  & 46.1$\pm{1.7}$& 72.6$\pm{0.8}$& 76.6$\pm{0.4}$ &63.7$\pm{0.4}$& 70.7$\pm{0.0}$& 72.5$\pm{0.1}$ &63.1$\pm{0.6}$ & 47.4$\pm{0.4}$ & 77.9$\pm{0.3}$ & 71.5$\pm{0.1}$ & 53.3$\pm{0.5}$ & 80.9$\pm{0.2}$& 66.4$\pm{0.2}$\\
PDA & 49.0 $\pm{0.4}$ & 69.6$\pm{1.0}$ & 85.1$\pm{0.8}$& 71.4$\pm{1.0}$ &64.6$\pm{0.5}$ & 81.0 $\pm{0.4}$ & 65.1$\pm{2.2}$ & 44.1$\pm{0.6}$&82.7$\pm{0.7}$& 75.9$\pm{0.4}$& 48.7$\pm{0.7}$& 80.3$\pm{0.3}$& 68.1$\pm{0.1}$\\
ODA  &64.1 $\pm{0.8}$& 84.1$\pm{0.1}$ & 88.3$\pm{0.3}$ & 76.7$\pm{0.4}$ & 80.7$\pm{0.8}$ & 84.9$\pm{0.5}$ & 77.6$\pm{0.5}$ & 62.7 $\pm{0.5}$& 85.4 $\pm{0.2}$& 80.8$\pm{0.6}$ & 65.1$\pm{0.4}$& 87.1$\pm{0.3}$& 78.1$\pm{0.1}$\\
OPDA & 64.1$\pm{1.8}$& 84.3$\pm{0.4}$& 91.2$\pm{0.5}$& 84.3$\pm{0.5}$& 78.3$\pm{0.6}$& 89.4$\pm{0.3}$& 83.4$\pm{1.1}$& 63.6$\pm{0.8}$& 91.4$\pm{0.5}$& 83.3$\pm{0.3}$& 63.9$\pm{0.3}$& 86.9$\pm{0.3}$& 80.4$\pm{0.1}$ \\
  \bottomrule[1.5pt]
\end{tabular}}
\caption{Standard deviation of DANCE in experiments on OfficeHome. The deviation is calculated by three runs. DANCE shows descent deviations.}
\label{tb:std_oh}
\end{center}
\end{table*}



\begin{table*}[]
\begin{center}

\scalebox{0.9}{
\begin{tabular}{c|cccccccc}
\toprule[1.5pt]
Setting  &A2W                    & D2W& W2D & A2D & D2A & W2A & Avg  & VD    \\\hline
CDA  & 88.6$\pm{0.4}$& 97.5$\pm{0.4}$& 100$\pm{0.0}$& 89.4$\pm{1.3}$& 69.5$\pm{1.5}$& 68.2$\pm{0.0}$& 85.5$\pm{0.2}$& 70.2$\pm{0.3}$\\
ODA  &93.6$\pm{2.3}$& 97.0$\pm{0.2}$& 97.1$\pm{0.5}$& 95.7$\pm{0.3}$& 91.0$\pm{0.8}$& 90.3$\pm{0.2}$& 94.1$\pm{2.5}$&65.3$\pm{2.3}$\\
OPDA &92.8$\pm{0.2}$&97.8$\pm{0.6}$&97.7$\pm{0.5}$& 91.6$\pm{1.9}$&92.2$\pm{0.1}$&91.4$\pm{0.4}$&93.9$\pm{0.3}$&69.2$\pm{0.6}$\\\hline \hline 
Setting  & A2C &W2C	&D2C& D2A & W2A& Avg & VD    \\\hline
PDA & 88.8$\pm{0.4}$& 79.2$\pm{0.3}$& 79.4$\pm{0.3}$& 83.7$\pm{3.3}$& 92.6$\pm{0.5}$& 84.8$\pm{1.5}$& 73.7$\pm{2.9}$\\

  \bottomrule[1.5pt]
\end{tabular}}
\caption{Standard deviation of DANCE in experiments on Office and VisDA. The deviation is calculated by three runs. DANCE shows descent deviations.}
\label{tb:std_office}
\end{center}
\end{table*}


\begin{table*}[]
\begin{center}

\scalebox{0.75}{
\begin{tabular}{c|c|ccccccccccccc}
\toprule[1.5pt]
Setting & Ablation &Ar2Cl                    & Ar2Pr & Ar2Rw & Cl2Ar & Cl2Pr & Cl2Rw & Pr2Ar & Pr2Cl & Pr2Rw & Rw2Ar & Rw2Cl & Rw2Pr & Avg      \\\hline
\multirow{2}{*}{Closed} & with memory                  & \bf{48.1}    & \bf{71.7}    & \bf{76.4}    & \bf{63.0}    & \bf{70.8}    & \bf{71.7}    & \bf{59.2}    & \bf{45.2}    & \bf{77.8}    & \bf{71.2}    & \bf{53.7}    & \bf{80.9} & \bf{65.8} \\
&w/o memory            & 26.0    & 68.3    & 75.2    & 62.3    & 68.0    & 69.5    & 59.1    & 41.1    & 75.8    & 71.0    & 48.3    & 80.3 & 62.1 \\\hline
%OH Partial                 &         &         &         &         &         &         &         &         &         &         &         &      &      \\\hline
\multirow{3}{*}{Partial} & with memory  &49.0 & 69.6 & 85.1 & 71.4 & 64.6 & 81.0 & 65.1 & 44.1 & 82.7 & 75.9 & 48.7 & 80.3 & 68.1 \\
&w/o memory            & 54.8    & 84.4    & 87.0    & 74.0    & 71.1    & 82.0    & 75.6    & 54.6    & 86.7    & 80.4    & 59.0    & 84.1 & 74.5 \\
&w/o memory, w/o rej & \bf{56.2}    & \bf{84.6}    & \bf{87.1}    & \bf{74.0}    & \bf{74.8}    & \bf{82.4}    & \bf{77.5}    & \bf{56.5}    & \bf{86.7}    & \bf{80.4}    & \bf{60.2}    & \bf{84.1} & \bf{75.4} \\
  \bottomrule[1.5pt]
\end{tabular}}
\caption{Ablation study on memory. This table corresponds to Table 9 in the main paper. ``w/o rej'' means the model does not have ``unknown'' sample rejection. Since partial DA does not have ``unknown'' samples, the performance improves.}
\label{tb:ab_memory}
\end{center}
\end{table*}


\begin{table}[]
 \begin{center}
 \scalebox{0.75}{
 \begin{tabular}{c|c|ccccccc}
 \toprule[1.5pt]
 %\\\hline
 Setting&Method&A2W & D2W & W2D&A2D&D2A&W2A&Avg\\\hline
 \multirow{2}{*}{Closed}&Jigsaw & 87.7 & \bf{98.7}  &\bf{100.0} & 84.5  &61.7&62.5      & 82.5\\
 &DANCE   &\bf{88.6} & 97.5 & \bf{100.0} & \bf{89.4} &\bf{69.5} & \bf{68.2} & \bf{85.5}\\\hline
% %\\\hline

 \multirow{2}{*}{Open}&Jigsaw & 89.4   & 95.5   & 93.6     & 93.8   & 90.3&89.3    & 92.0 \\
&DANCE   & \bf{93.6} & \bf{97.0} & \bf{97.1} & \bf{95.7} & \bf{91.0} & \bf{90.3} & \bf{94.1}
 \\
 \bottomrule[1.5pt]
 \end{tabular}}
  \vspace{-4mm}
 \caption{Comparison between jigsaw \cite{carlucci2019domain,noroozi2016unsupervised} and DANCE on the Office dataset. For a fair comparison, we replace the loss of entropy similarity with jigsaw puzzle loss.}
\label{tb:jigsaw}
 \end{center}
 \end{table}



\begin{figure*}[t]

\begin{subfigure}[b]{0.32\textwidth}
  \begin{center}
   \includegraphics[width=\textwidth]{imgs/vary_lambda.png}
    \caption{Value of $\lambda$ in Eq. 9.}
     \label{fig:change_lambda}
  \end{center}
 \end{subfigure}
 ~ 
 \begin{subfigure}[b]{0.32\textwidth}
  \begin{center}
   \includegraphics[width=\textwidth]{imgs/vary_margin.png}
    \caption{Value of $m$ in Eq. 7.}
    \label{fig:change_margin}
  \end{center}
 \end{subfigure}
 ~ 
 \begin{subfigure}[b]{0.32\textwidth}
  \begin{center}
   \includegraphics[width=\textwidth]{imgs/vary_separation.png}
    \caption{Value of $\rho$ in Eq. 7.}
     \label{fig:change_separation}
  \end{center}
 \end{subfigure}
 ~ 
 \vspace{-3mm}
  \caption{(a): Varying the value of $\lambda$ in Eq. 9. (b): Varying the value of margin in Eq. 7. (c): Varying the value of $\rho$ in Eq. 7, which is determined based on the number of known classes. }
  % (Real to Clipart in DomainNet). \bf{Left}: Alexnet, \bf{Right}: VGG.
   %\label{fig:change_unk}
   \label{fig:hyperparameters}
\end{figure*}

\section{Dataset Detail}
In PDA, 10 classes in Caltech-256 are used as shared classes $(L_s \cap L_t)$. The other 21 classes are used as source private classes $(L_s - L_t)$. %\donghyun{Check the notation $L_cm,L_c$, as we changed the meaning of the notation.} 
Since DSLR and Webcam do not have many examples, we conduct experiments on D to A, W to A, A to C (Caltech), D to C, and W to C shifts. 
In OSDA, the same 10 classes are used as shared classes $(L_s \cap L_t)$ and the selected 11 classes are used as unknown classes $(L_t - L_s)$. The setting is the same as \cite{saito2018open}. In OPDA, the same 10 class are used as shared classes $(L_s \cap L_t)$ and then, in alphabetical order, the next 10 classes are used as source private classes $(L_s - L_t)$, and the remaining 11 classes are used as unknown classes $(L_t - L_s)$. The second benchmark dataset is \textbf{OfficeHome (OH)}~\cite{venkateswara2017Deep}, which contains four domains and 65 classes. In PDA, in alphabetical order, the first 25 classes are selected as shared classes $(L_s \cap L_t)$ and the rest classes are source private classes $(L_s - L_t)$. In OSDA, the first 15 classes are used as shared classes $(L_s \cap L_t)$ and the rest classes are used as unknown classes $(L_t - L_s)$. In OPDA, the first 10 classes are used as shared classes $(L_s \cap L_t)$, the next 5 classes are source private classes $(L_s - L_t)$ and the rest are unknown classes $(L_t - L_s)$. The third dataset is \textbf{VisDA}~\cite{peng2017visda}, which contains 12 classes from the two domains, synthetic and real images. The synthetic domain consists of 152,397 synthetic 2D renderings of 3D objects and the real domain consists of 55,388 real images. 
In PDA, the first 6 classes are used as shared classes $(L_s \cap L_t)$ and the rest are source private classes $(L_s - L_t)$. In OSDA, we follow \cite{saito2018open} and use the 6 classes as shared classes $|L_s \cap L_t|$ and the rest as unknown classes $(L_t - L_t)$. In OPDA, the first 6 classes are shared classes $(L_s \cap L_t)$, the next 3 are source private classes $(L_s - L_t)$ and the other 3 classes are unknown classes $(L_t - L_s)$. We mainly perform experiments on these three datasets with four settings because it enables direct comparison with many state-of-the-art results. We provide an analysis of varying the number of classes using Caltech~\cite{griffin2007caltech} and ImageNet~\cite{imagenet} because these datasets contain a large number of classes.


% \section{Dataset Detail}
% In PDA, 10 classes which are shared with Caltech-256 are used as $|L_s \cap L_t|$. The other 21 classes are used as $|L_s - L_t|$. %\donghyun{Check the notation $L_cm,L_c$, as we changed the meaning of the notation.} 
% Since DSLR and Webcam do not have many examples, we conduct experiments on D to A, W to A, A to C (Caltech), D to C, and W to C shifts. 
% In OSDA, the same 10 classes are used as $|L_s \cap L_t|$ and the selected 11 classes are used as $|L_t - L_s|$. The setting is the same as \cite{saito2018open}. In OPDA, the same 10 class are used as $|L_s \cap L_t|$ and then, in alphabetical order, the next 10 classes are used as $|L_s - L_t|$, and the remaining 11 classes are used as $|L_t - L_s|$. The second benchmark dataset is \textbf{OfficeHome (OH)}~\cite{venkateswara2017Deep}, which contains four domains and 65 classes. In PDA, in alphabetical order, the first 25 classes are selected as $|L_s \cap L_t|$ and rest classes are $|L_s - L_t|$. In OSDA, the first 15 classes are used as $|L_s \cap L_t|$ and rest classes are $L_t$. In OPDA, the first 10 classes are used as $|L_s \cap L_t|$, next 5 classes are $|L_s - L_t|$ and rest are $|L_t - L_s|$. The third dataset is \textbf{VisDA}~\cite{peng2017visda}, which contains 12 classes from the two domains, synthetic and real images. The synthetic domain consists of 152,397 synthetic 2D renderings of 3D objects and the real domain consists of 55,388 real images. 
% In PDA, the first 6 classes are used as $|L_s \cap L_t|$ and rest are $|L_s - L_t|$. In OSDA, we follow \cite{saito2018open} and use 6 classes as $|L_s \cap L_t|$ and rest as $L_t$. In OPDA, the first 6 classes are $|L_s \cap L_t|$, the next 3 are $|L_s - L_t|$ and the other 3 classes are $|L_t - L_s|$. We mainly perform experiments on these three datasets with four settings because it enables direct comparison with many state-of-the-art results. We provide an analysis of varying the number of classes using Caltech~\cite{griffin2007caltech} and ImageNet~\cite{imagenet} because these datasets contain a large number of classes.

\section{Implementation Detail}
We list the implementation details which are excluded from the main paper due to a limit of space. 


\textbf{DANCE (universal comparison).}
The batch-size is set as 36. The temperature parameter in Eq. 5 is set as 0.05 by following~\cite{saito2019semi}. We train a model for 10,000 iterations with nestrov momentum SGD and report the performance at the end of the iterations. 
The initial learning rate is set as $0.01$, which is decayed with the factor of $(1 + \gamma \frac{i}{10,000})^{-p}$, where $i$ denotes the number of iterations and we set $\gamma = 10$ and $p=0.75$. The learning rate of pre-trained layers is multiplied by $0.1$. We follow \cite{saito2019semi} for this scheduling method.

\textbf{Baselines (universal comparison).}
We use the following released codes for ETN~\cite{ETN_2019_CVPR}(\url{https://github.com/thuml/ETN}), UAN~\cite{UDA_2019_CVPR}(\url{https://github.com/thuml/Universal-Domain-Adaptation}),  and STA~\cite{Liu_2019_CVPR}(\url{https://github.com/thuml/Separate_to_Adapt}). We tune the hyper-parameter of these methods by validating the performance on OPDA, Amazon to DSLR, Office. Since we could not see improvements by changing the hyper-parameters from their codes, we employed the hyper-parameters provided in their codes. For ETN, we use the hyper-parameters for Office-Home. For UAN and STA, we use the hyper-parameters for Office. We implement DANN by ourselves and tuned the hyper-parameters by the performance on OPDA, Amazon to DSLR, Office. For all of these methods, we report the performance at the end of training for comparison. We observe that there is a gap in the performance between the best checkpoint and the final checkpoint. This can explain the gap between the reported performance in their paper and the performance in our universal comparisons. 
%\donghyun{it needs to synchronize with present tense, I changed some but need to be checked again.}


\textbf{Ours (non-universal comparison).}
In the non-universal comparison, we have prior knowledge about the class distribution in the target domain. For example, we know that there are no ``unknown'' samples in PDA and CDA. Therefore, we do not have to consider ``unknown'' sample rejection both in a training and testing phase. We will include the parameters used in this comparison when we publish a code. 

\textbf{Baselines (non-universal comparison).}
We run experiments for STA (OfficeHome ODA) and ETN (A2C, W2C, D2C, PDA) since the results are not available in their papers. For STA, we tune the hyper-parameters of a trade-off of the entropy. We could see an improvement on average. For ETN, we report the performance which employs the same hyper-parameters as the universal comparison but does not use ``unknown'' sample rejection. 
For other non-universal comparisons, we show the performance of the results reported in their papers. ``NA'' indicates the results are not available in their paper. 
We observe the performance gap in our universal comparison and the reported performance in each paper. For example, the performance of UAN in OPDA has a big gap between the universal comparison and the non-universal comparison (reported accuracy) although we use the same hyper-parameters. We could obtain similar performance to the reported number if we pick up the best checkpoint for each setting. But, we report the performance of fixed iterations' checkpoints for a fair comparison, which can explain the gap.

\section{Supplemental Results}
%\donghyun{making the best number bold in tables}
\textbf{Detailed results of ODA and OPDA.}
Table \ref{tb:oda_opada} shows the detailed results of ODA and OPDA. OS* shows the averaged accuracy over known classes while OS shows the averaged accuracy including unknown class. DANCE shows good performance on both metrics. ETN shows better results on OS* than DANCE in several scenarios. In ETN results, OS* shows much better results on OS, which means that ETN is not good at recognizing unknown samples as unknown. This is clearly shown in Figure 6 (c) in our main paper. 


\textbf{Comparison with Jigsaw~\cite{carlucci2019domain}.}
Table \ref{tb:jigsaw} shows the comparison with jigsaw puzzle based self-supervised learning. To consider the self-supervised learning part of DANCE, we replaced neighborhood clustering loss with the jigsaw puzzle loss on the target domain. The jigsaw puzzle loss is calculated on target samples. We can see that DANCE performed better in almost all settings and confirm the effectiveness of clustering based self-supervision for this task.

\textbf{Results with standard deviations.}
Table \ref{tb:std_oh} and \label{tb:std_office} show results of DANCE with standard deviations. We show only the averaged accuracy over three runs in the main paper due to a limit of space. We show the standard deviation. We can observe that DANCE shows decent standard deviations. 


\textbf{Detailed results of non-universal comparison.}
Table \ref{tb:ab_memory} shows detailed results of the non-universal comparison in PDA OfficeHome and Table 9 in our main paper. As we explain in our main paper, by ablating the memory features, we could see much change in the performance in some settings. 
Besides, since the two settings do not include unknown target samples, we can see improvement by ablating unknown sample rejection in the test phase (74.5 to 75.4 on average in Partial). 


\textbf{Sensitivity to hyper-parameters.}
In Fig.~\ref{fig:hyperparameters}, we show the sensitivity to hyper-parameters on OPDA setting of Amazon to DSLR, which we used to tune the hyper-parameters. Although $\rho$ in Eq. 5 is decided based on the number of source classes, we show the behavior of our method when changing it in Fig. \ref{fig:change_separation}. When we increase the value, more examples will be decided as known, then the performance on unknown examples decreases. 


==> tables/ablation.tex <==

\begin{table}[t]
\begin{center}
\scalebox{0.85}{
\begin{tabular}{c|ccccccc}
\toprule[1.5pt]
Ablation&A2W & D2W & W2D&A2D&D2A&W2A&Avg\\\hline
w/o NC& 72.8&96.2& \bf{100.0}&75.3&35.7& 54.8 & 72.5\\
w/o ES&78.5&95.7&99.8&78.7& \bf{69.5} & 68.0 & 81.7\\
FULL  &\bf{88.6} & \bf{97.5} & \bf{100.0} & \bf{89.4} & \bf{69.5} & \bf{68.2} & \bf{85.5}\\
\bottomrule[1.5pt]
\end{tabular}}
\caption{\small Ablation study on Neighborhood Clustering (NC) and the entropy separation (ES).}
\label{tb:ab2}
\end{center}
\end{table}

==> tables/ablation_cluster.tex <==
\begin{table}[t!]
\vspace{-3mm}
  \begin{minipage}[t]{.45\textwidth}
     \addtolength{\tabcolsep}{-3pt}
     \caption{\small 
     %Analysis of ability to cluster ``unknown '' class samples. 
     DANCE provides better representations for classifying ``unknown'' class examples into their classes.}
     \vspace{-2mm}
    \begin{center}
    \scalebox{0.75}{
    \begin{tabular}[t]{l|ccccc}
\toprule[1.5pt]
Method &D to A & W to A & R to P & R to C&VisDA\\\hline
ImgNet &44.6&44.6&56.4&17.4&73.2\\
SO     & 53.5       & 54.1 &58.2&20.7&72.3 \\
DANN   & 50.9       & 52.2 &44.1&14.9&50.2 \\
DANCE   & \bf{57.5} & \bf{57.4}&\bf{63.5}&\bf{22.8}&\bf{75.2}\\
 \bottomrule[1.5pt]
\end{tabular}}
 \end{center}
%\vspace{-7mm}
\label{tb:fewshot}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{.45\textwidth}
   \addtolength{\tabcolsep}{-3pt}  
   \caption{\small Ablation study of Neighborhood Clustering (NC) and entropy separation (ES).} \vspace{-3mm}
    \begin{center}
    \scalebox{0.8}{
\begin{tabular}[t]{c|ccccccc}
\toprule[1.5pt]
Ablation&A2W & D2W & W2D&A2D&D2A&W2A&Avg\\\hline
w/o NC& 72.8&96.2& \bf{100.0}&75.3&61.9& 54.8 & 76.8\\
w/o ES&78.5&95.7&99.8&78.7& 68.9 & 68.0 & 81.7\\
FULL  &\bf{88.6} & \bf{97.5} & \bf{100.0} & \bf{89.4} & \bf{69.5} & \bf{68.2} & \bf{85.5}\\
\bottomrule[1.5pt]
\end{tabular}}
 \end{center}
\label{tb:ab2}
  \end{minipage}
  \vspace{-6mm}
\end{table}

==> tables/class_list.tex <==

\begin{table}[t]
\begin{center}

\scalebox{0.9}{
\begin{tabular}{l|cccc}
\toprule[1.5pt]
\multirow{2}{*}{Dataset} &\multicolumn{4}{c}{Class Split ($|L_s \cap L_t | / |L_s - L_t | / |L_t - L_s|$)}\\
 &CDA & PDA & ODA &OPDA\\\hline
Office &31 / 0 / 0&10 / 21 / 0&10 / 0 / 11&10 / 10 / 11\\
OH &65 / 0 / 0&25 / 40 / 0&15 / 0 / 50&10 / 5 / 50\\
VisDA  &12 / 0 / 0&6 / 6 / 0&6 / 0 / 6&6 / 3 / 3 \\
 \bottomrule[1.5pt]
\end{tabular}}
\caption{The number of shared / source private / target private classes in each setting. }
\label{tb:class_split}
\end{center}
\end{table}


==> tables/deviation_officehome.tex <==

\begin{table*}[t]
\begin{center}

\scalebox{0.7}{
\begin{tabular}{c|ccccccccccccc}
\toprule[1.5pt]
Setting  &Ar2Cl                    & Ar2Pr & Ar2Rw & Cl2Ar & Cl2Pr & Cl2Rw & Pr2Ar & Pr2Cl & Pr2Rw & Rw2Ar & Rw2Cl & Rw2Pr & Avg      \\\hline
CDA  & 54.0$\pm{0.7}$& 75.8$\pm{0.8}$& 78.2$\pm{0.5}$ &64.8$\pm{0.5}$& 72.2$\pm{0.4}$& 73.6$\pm{0.1}$ &63.0$\pm{0.6}$ & 53.1$\pm{0.4}$ & 79.3$\pm{0.4}$ & 72.8$\pm{0.2}$ & 58.1$\pm{0.6}$ & 82.8$\pm{0.3}$& 69.1$\pm{0.2}$\\
PDA & 53.6 $\pm{0.3}$ & 73.2$\pm{0.8}$ & 84.9$\pm{0.8}$& 70.8$\pm{0.8}$ &67.3$\pm{0.7}$ & 82.6 $\pm{0.3}$ & 70.0$\pm{1.2}$ & 50.9$\pm{0.7}$&84.8$\pm{0.7}$& 77.0$\pm{0.2}$& 55.9$\pm{0.9}$& 81.8$\pm{0.4}$& 71.1$\pm{0.1}$\\
ODA  &64.1 $\pm{0.8}$& 84.1$\pm{0.1}$ & 88.3$\pm{0.3}$ & 76.7$\pm{0.4}$ & 80.7$\pm{0.8}$ & 84.9$\pm{0.5}$ & 77.6$\pm{0.5}$ & 62.7 $\pm{0.5}$& 85.4 $\pm{0.2}$& 80.8$\pm{0.6}$ & 65.1$\pm{0.4}$& 87.1$\pm{0.3}$& 78.1$\pm{0.1}$\\
OPDA & 64.1$\pm{1.8}$& 84.3$\pm{0.4}$& 91.2$\pm{0.5}$& 84.3$\pm{0.5}$& 78.3$\pm{0.6}$& 89.4$\pm{0.3}$& 83.4$\pm{1.1}$& 63.6$\pm{0.8}$& 91.4$\pm{0.5}$& 83.3$\pm{0.3}$& 63.9$\pm{0.3}$& 86.9$\pm{0.3}$& 80.4$\pm{0.1}$ \\
  \bottomrule[1.5pt]
\end{tabular}}
\caption{Standard deviation of DANCE in experiments on OfficeHome. The deviation is calculated by three runs. DANCE shows descent deviations.}
\label{tb:std_oh}
\end{center}
\end{table*}


==> tables/memory.tex <==

\begin{table}[t]
\begin{center}
\scalebox{0.85}{
\begin{tabular}{c|c|ccc}
\toprule[1.5pt]
Setting & Ablation & OH & Office  & VisDA  \\\hline
\multirow{2}{*}{Closed} & with memory  & \bf{66.4} &85.5 &70.2\\
&w/o memory            & 62.1 & 85.5& \bf{70.5}\\\hline

\multirow{2}{*}{Partial} & with memory  & 68.1 &84.8 & \bf{73.7}\\
&w/o memory            &  \bf{74.5} &  \bf{88.4}&69.4\\
  \bottomrule[1.5pt]
\end{tabular}}
 \vspace{-3mm}
\caption{Ablation study on memory using Office-Home (OH) and Office. Additional results can be found in supplementary.}
\vspace{-3mm}
\label{tb:ab_memory}
\end{center}
\end{table}
